Behavioural types for non-uniform memory accesses

Concurrent programs executing on NUMA architectures consist of concurrent entities (e.g. threads, actors) and data placed on different nodes. Execution of these concurrent entities often reads or updates states from remote nodes. The performance of such systems depends on the extent to which the concurrent entities can be executing in parallel, and on the amount of the remote reads and writes. We consider an actor-based object oriented language, and propose a type system which expresses the topology of the program (the placement of the actors and data on the nodes), and an effect system which characterises remote reads and writes (in terms of which node reads/writes from which other nodes). We use a variant of ownership types for the topology, and a combination of behavioural and ownership types for the effect system.

==> eptcsdata.tex <==
\providecommand{\firstpage}{109}
\providecommand{\publicationstatus}{S. J. Gay and J. Alglave (Eds.): Programming Language Approaches to\\ Concurrency- and Communication-Centric Software (PLACES 2015).\\
EPTCS 203, 2016, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.203.9}{10.4204/EPTCS.203.9}}
\pdfoutput=1

